AmbigQA: Answering Ambiguous Open-domain Questions

Ambiguity is inherent to open-domain question answering; especially when exploring new topics, it can be difficult to ask questions that have a single, unambiguous answer. In this paper, we introduce AmbigQA, a new open-domain question answering task which involves finding every plausible answer, and then rewriting the question for each one to resolve the ambiguity. To study this task, we construct AmbigNQ, a dataset covering 14,042 questions from NQ-open, an existing open-domain QA benchmark. We find that over half of the questions in NQ-open are ambiguous, with diverse sources of ambiguity such as event and entity references. We also present strong baseline models for AmbigQA which we show benefit from weakly supervised learning that incorporates NQ-open, strongly suggesting our new task and data will support significant future research effort. Our data and baselines are available at https://nlp.cs.washington.edu/ambigqa.

==> Sections/14-zero-shot.tex <==
% MOVED THIS TO SECTION 6


%\subsection{Zero-shot \answerprediction}
Since \dataname\ provides an evaluation set with explicit sets of multiple answers, we can also test if models trained on partial supervision only (\nqopen) are capable of producing full answer sets.
This may be important for modeling in domains where single-answer datasets are available but full annotations like in \dataname\ are not.
%We can use thresholding as described in Section~\ref{subsec:baselines} to decode multiple answers from models trained only on \nqopen.
%In addition to the standard setting, we present a zero-shot setting where a system predicts multiple distinct answers without using \dataname\ training data.
To this end, we present a zero-shot setting where a system predicts multiple distinct answers without using \dataname\ training data.
We include four \nqopen\ models including ours, consisting of diverse approaches and model architectures, as baselines.
These models, when trained on \nqopen, may be made to predict multiple answers via thresholding as described in Section~\ref{subsec:baselines}.\footnote{
    We allow using \dev\ data to tune the threshold $\gamma$,
    although this arguably makes our setting not zero-shot in the strictest sense.
    %; we call this setting zero-shot for convenience.
} 
Table~\ref{tab:zero-shot-result} reports zero-shot performance.
Although \citet{min2019knowledge} outperforms \citet{asai2019learning} on \nqopen, it is worse on \dataname.
In addition, although \modelname\ outperforms \citet{karpukhin2020dense} in the standard setting, it is worse in zero-shot \Fanswer\ ({\em multi}),
potentially because thresholding exacerbates the problems that \modelname\ has with long sequences (Section~\ref{subsec:main-results}).
%presumably because we use the perplexity of the answer sequence for thresholding but perplexity does not correlate well with the likelihood of the answer.
%\footnote{We observe the perplexity of the answer sequence does not correlate with the accuracy of answers, in both standard QA setting and \taskname\ setting. We leave it for future work to find an alternative way to compute the likelihood of the answer in the sequence-to-sequence model. }
%\julian{I think it wouldn't occur to the reader that we should train question disambiguation on NQ-open, we probably don't need to say the below.}
%Note that, although it is possible to obtain \Fedit\ from the QG model trained on \nqopen, the numbers are significantly low ($3.7$ \Fanswer\ on the \dev\ data with \modelname), as generating the question on \nqopen\ is not for differentiating distinct answers.

\begin{table}
    \centering \footnotesize
	\begin{tabular}{l P{1.05cm} P{0.6cm} P{0.6cm} }
    \toprule
        \multirow{2}{*}{Model} &
        {\scriptsize \nqopen} EM & \Fanswer\ (\em all) & \Fanswer\ (\em multi) \\
    \midrule
        \multicolumn{4}{l}{\textbf{\em Dev}} \\
        \citet{min2019knowledge} & 34.7 & 30.8 & 20.4 \\ % 38.9
        \citet{asai2019learning} & 31.7 & 29.7 & 19.7 \\ % 37.7
        \citet{karpukhin2020dense} & 39.8 & 35.2 & \tf{26.5} \\ % 38.0->46.0
        \modelname & \tf{42.0} & \tf{36.4} & 24.8 \\ % 39.3->48.2
    \midrule
        \multicolumn{4}{l}{\textbf{\em Test}} \\
        \citet{min2019knowledge} & 34.5 & 27.5 & 17.0 \\ % 33.4
        \citet{asai2019learning} & 32.6 & 27.9 & 17.7 \\ % 34.4
        \citet{karpukhin2020dense} & {41.5} & {30.1} & \tf{23.2} \\ % 38.1->38.6
        \modelname & \tf{42.2} & \tf{30.8} & 20.7 \\ % 40.0->42.4
    \bottomrule
    \end{tabular}
	\caption{
	    Zero-shot performance on \answerprediction\ of the models trained on \nqopen.
	    We report Exact Match (EM) on \nqopen\ and \Fanswer\ on \dataname.
	}\label{tab:zero-shot-result}
\end{table}
